The Parallel Reversible Pebbling Game: Analyzing the Post-Quantum Security of iMHFs

The classical (parallel) black pebbling game is a useful abstraction which allows us to analyze the resources (space, space-time, cumulative space) necessary to evaluate a function $f$ with a static data-dependency graph $G$. Of particular interest in the field of cryptography are data-independent memory-hard functions $f_{G,H}$ which are defined by a directed acyclic graph (DAG) $G$ and a cryptographic hash function $H$. The pebbling complexity of the graph $G$ characterizes the amortized cost of evaluating $f_{G,H}$ multiple times as well as the total cost to run a brute-force preimage attack over a fixed domain $\mathcal{X}$, i.e., given $y \in \{0,1\}^*$ find $x \in \mathcal{X}$ such that $f_{G,H}(x)=y$. While a classical attacker will need to evaluate the function $f_{G,H}$ at least $m=|\mathcal{X}|$ times a quantum attacker running Grover's algorithm only requires $\mathcal{O}(\sqrt{m})$ blackbox calls to a quantum circuit $C_{G,H}$ evaluating the function $f_{G,H}$. Thus, to analyze the cost of a quantum attack it is crucial to understand the space-time cost (equivalently width times depth) of the quantum circuit $C_{G,H}$. We first observe that a legal black pebbling strategy for the graph $G$ does not necessarily imply the existence of a quantum circuit with comparable complexity -- in contrast to the classical setting where any efficient pebbling strategy for $G$ corresponds to an algorithm with comparable complexity evaluating $f_{G,H}$. Motivated by this observation we introduce a new parallel reversible pebbling game which captures additional restrictions imposed by the No-Deletion Theorem in Quantum Computing. We apply our new reversible pebbling game to analyze the reversible space-time complexity of several important graphs: Line Graphs, Argon2i-A, Argon2i-B, and DRSample. (See the paper for the full abstract.)

==> ec-prelim.tex <==
% !TEX root = tcc-main.tex
\ignore{\section{Preliminaries}
\seclab{sec:prelim}



\subsection{Graph Notations and Definitions}
\seclab{sec:prelim:graph}



\subsection{(Classical) Graph Pebbling Games}
\seclab{sec:prelim:pebbling}

Here, we recall the parallel (and sequential) pebbling games played over a directed acyclic graph which are the main computational models for analyzing memory-hard functions used in a number of studies \cite{STOC:AlwSer15,EC:AlwBloPie17,EC:AlwBloPie18,C:BHKLXZ19,ITCS:BloLeeZho20,ITCS:AmeBloZho20}.

The goal of the (classical) pebbling game is to place pebbles on all the target nodes of some input DAG $G=(V,E)$. The game proceeds in rounds, and each round $i$ consists of a number of pebbles $P_i\subseteq V$ which we call a \emph{pebbling configuration} at round $i$. The game must satisfy the following constraints: initially, the graph is unpebbled, i.e., $P_0 = \varnothing$. In each round $i\geq 1$, we can place a pebble on $v\in P_i$ only if either $v$ contained a pebble in the previous round $(v\in P_{i-1})$ or all of its parents were pebbled in the previous round $(\parents(v,G)\subseteq P_{i-1})$. In a sequential pebbling game, we require an additional condition that at most one new pebble can be placed in any round, i.e., $|P_i\setminus P_{i-1}|\leq 1$. Otherwise, we call the game as a parallel pebbling game. }
